VepAgent: Bridging Causal-Transition via Tool-Augmented Reinforcement Learning for Video Event Prediction

Multimodal Large Language Models (MLLMs) have demonstrated remarkable potential in video understanding, yet their reliance on retrospective summarization and text-centric priors often limits their ability to bridge unobserved causal transitions when applied to Video Event Prediction (VEP). To address this, we propose VepAgent, an agentic framework that integrates causal-transition reasoning with tool-augmented reinforcement learning (RL) for robust VEP. Unlike prior methods that passively project future trajectories from historical dependencies, our approach explicitly models the logical progression from terminal observed states to future events. Specifically, we first construct futurebench-4K, a high-quality chain-of-thought dataset for supervised fine-tuning (SFT) that effectively bridges the causal-logic gap by structuring the deduction of unobserved intermediate states. Subsequently, we develop a diagnostic tool library integrating state tracking, frame retrieval, and region magnification, enabling the agent to dynamically augment reasoning with external tools to recover missing spatio-temporal evidence and resolve visual ambiguities during inference. Moreover, we propose a composite reward mechanism that jointly optimizes prediction accuracy, causal coherence, and reliable prior, compelling the agent to rely on genuine visual grounding rather than superficial textual similarities. Extensive evaluations on FutureBench and NEPBench datasets demonstrate that our method achieves state-of-the-art performance, significantly outperforming larger MLLMs and validating the empirical effectiveness of our agentic, future-oriented reasoning paradigm.

==> One_Equation.tex <==
\textbf{Reward Design.} Effective reward functions should balance prediction accuracy, causal-logic bridging, and robustness against language-prior shortcuts. To this end, we design a composite reward that integrates three components: an accuracy reward $R_{\text{Acc}}$, a causal gap reward $R_{\text{Gap}}$, and an anti-prior reward $R_{\text{AntiPrior}}$, all gated by a format reward $R_{\text{Format}}$. The final reward is formally defined as:
\begin{equation}
R(\tau) = R_{\text{Format}}(\tau) \cdot \left( 0.65 R_{\text{Acc}}(\tau) + 0.20 R_{\text{Gap}}(\tau) + 0.15 R_{\text{AntiPrior}}(\tau) \right).
\label{eq:total_reward}
\end{equation}

The format reward serves as a hard gate to ensure structural coherence, where $R_{\text{Format}}(\tau)=1$ if the trajectory $\tau$ strictly follows the required reasoning format (e.g., containing valid \textit{<thinking>} and \textit{<answer>} tags), and $0$ otherwise. Any trajectory failing this check receives zero overall reward to prevent reward manipulation. The accuracy reward $R_{\text{Acc}}$ is a binary metric quantifying the correctness of the final prediction, where $R_{\text{Acc}}(\tau)=1$ if the predicted future event $y_p$ semantically matches the ground-truth event $y_g$ (e.g., via cosine similarity above a threshold), and $0$ otherwise.

Differently, the causal gap reward $R_{\text{Gap}}$ quantifies whether the model's reasoning genuinely bridges the unobserved intermediate state transition rather than directly guessing the future. It requires the reasoning chain $z$ to satisfy two conditions: (1) \textbf{Semantic Coherence}, where the reasoning content aligns with the ground-truth event $y_g$, and (2) \textbf{Causal Progression}, where the reasoning explicitly articulates the logical progression from the terminal observed state and ongoing action toward the future result. If both conditions are met, $R_{\text{Gap}}(\tau)=1$; otherwise, it is $0$.

Furthermore, the anti-prior reward $R_{\text{AntiPrior}}$ is designed to mitigate the language-prior shortcut, where models merely select the option with the highest textual similarity to the query $Q$. For a given query and the correct option among $K$ candidates, we compute the textual similarity rank $k$ of the correct option with respect to $Q$. If the model predicts correctly ($R_{\text{Acc}}=1$), we assign a higher reward when the correct option is less textually guessable (i.e., a larger rank $k$). The reward is defined as $R_{\text{AntiPrior}}(\tau) = \frac{k - 1}{K - 1}$ (yielding $0$ for the most obvious guess and $1$ for the least obvious), and $0$ if the prediction is incorrect. This continuous formulation strongly incentivizes the agent to rely on visual evidence rather than superficial textual priors. Such a composite reward not only maximizes prediction accuracy but also enforces causal bridging and penalizes language shortcut behaviors.

